Beyond Time Shifts: Adapting Omni-LLM as a Reference-Free Evaluator for Generative Audio-Visual Models

As audio-visual generative models evolve into world simulators, cross-modal synchronization stands as a critical proxy for assessing the consistency of world dynamics and causality in generated content. However, existing evaluation metrics presume structural correctness, reducing synchronization to mere temporal alignment. Consequently, they fail on generative outputs, especially when exhibiting structural hallucinations and asymmetric cross-modal relations, which currently \textbf{mandate expert human annotation to assess synchronization.} This dependency introduces a critical paradox: \emph{human evaluators rely on relative, reference-dependent comparisons, whereas automated metrics require reference-free, absolute scalars.} We resolve this paradox by proposing a framework that distills relative human perception into a continuous, globally consistent metric. First, we introduce SynthSync, a dataset of generative failures ranked via pairwise human annotations. Second, we adapt the Omni-LLM equipped with a continuous latent projection to translate relative human rankings into continuous absolute values. Third, we propose Real-Valued Group Relative Policy Optimization ($\mathbb{R}$-GRPO) to internalize the global causal structure of synchronization via listwise score distributions. Empirically, our metric achieves state-of-the-art human preference alignment. We leverage this estimator to establish a standardized benchmark, advancing AV-Gen assessment from low-level signal correlation to visually grounded causality.

==> Tables/LTX2BoN.tex <==
\begin{table}[]
\begin{tabular}{|c|c|c|c|}
\hline
BoN Reward   & AV-Align                       & JavisScore                     & Our Metric                     \\ \hline
Random       & 0.0698                         & 0.0714                         & 0.8820                         \\ \hline
+AV-Align    & \cellcolor[HTML]{EFEFEF}0.2116 & 0.0710                         & \textbf{3.2385}                \\ \hline
+ JavisScore & 0.0725                         & \cellcolor[HTML]{EFEFEF}0.1633 & 1.7417                         \\ \hline
+ Ours       & \textbf{0.1439}                & \textbf{0.0934}                & \cellcolor[HTML]{EFEFEF}5.0589 \\ \hline
\end{tabular}
\end{table}


==> Tables/TrainSetSta.tex <==
\begin{table}[]
\begin{tabular}{|c|c|c|c|}
\hline
Event Concept      & Sample Ratio () & \# Category & Category Examples                             \\ \hline
Animal Sound       & 29.6            & 52          & dog barks, bird crows, lion roaring, ....     \\ \hline
Musical Intruments & 5.5             & 58          & guitar, piano, drum, ...                      \\ \hline
Human Sounds       & 5.6             & 25          & clapping, cheering, screaming, ...            \\ \hline
Vehicle            & 23.9            & 15          & car engine, helicopter, train siren, ...      \\ \hline
Natural Sound      & 8.2             & 15          & rain, thunder wind, ocean waves, ...          \\ \hline
Sports             & 4.9             & 15          & basketball bounce, golf, tennis, ...          \\ \hline
Machine Sound      & 18.7            & 20          & vacuum cleaner, hair dryer, door slamming,... \\ \hline
Miscellaneous      & 3.6             & 20          & fireworks, church bells, alarm clock, ...     \\ \hline
\end{tabular}
\end{table}


==> outline.tex <==
1. We have entered the era of hyper-realistic video generation (Sora, Veo 3). Yet, the illusion of reality shatters the moment sound is introduced. Why? Because true audio-visual synchronization is not just a signal processing problem; it is a test of multimodal physics. Currently, the field is flying blind. We cannot optimize what we cannot measure, and our inability to computationally evaluate general-scene synchronization is the primary bottleneck preventing the next leap in embodied multimodal generation.

2. 
Welcome to the brainstorming room. Grab a coffee. As a team of senior researchers who have spent years thinking about scaling laws, multimodal alignment, and the future of models like Gemini, Veo, and Sora, we are going to tell you the hard truth: Your current narrative is a chronological lab report. It tells the reviewer what you did, but it utterly fails to tell them why it changes the world.
To win a Best Paper at NeurIPS, you don't just present a better tool; you present a paradigm shift. You need to elevate your paper from "we built a better evaluation metric" to "we solved a fundamental bottleneck in multimodal AGI and introduced a novel RL paradigm to do it."
Here is how we at DeepMind would restructure your narrative to make a NeurIPS Meta-Reviewer sit up in their chair.
The DeepMind Narrative: "From Signal Processing to Semantic Reasoning"
Title Concept:
Something punchy that hints at the paradigm shift. e.g.,
"Hearing What You See: Evaluating General Audio-Visual Synchronization via Continuous RL in Omni-Models" OR "Beyond Offsets: Aligning Multimodal Physics with Omni-LLM Generative Reward Models"
Act 1: The "Sora/Veo Bottleneck" (The Grand Vision)
Instead of: "There lacks a sophisticated method to evaluate sync..."
Say: "We have entered the era of hyper-realistic video generation (Sora, Veo 3). Yet, the illusion of reality shatters the moment sound is introduced. Why? Because true audio-visual synchronization is not just a signal processing problem; it is a test of multimodal physics. Currently, the field is flying blind. We cannot optimize what we cannot measure, and our inability to computationally evaluate general-scene synchronization is the primary bottleneck preventing the next leap in embodied multimodal generation."
Act 2: The "Semantic Grounding" Paradigm Shift (Literature Review as a Weapon)
Instead of listing what previous models can't do, group them into "eras" and show why they are fundamentally obsolete.
Era 1: Domain-Specific & Linear (The past): Lip-sync metrics or Synchformer. They treat video as a linear timeline to be shifted. They have no concept of what is happening.
Era 2: Heuristic & Repetitive (The band-aid): AV-Align relies on onset-detection (beats, impacts). It fails on continuous, non-percussive sounds.
Era 3: Contrastive & Spatially Blind (The false dawn): JavisScore (ImageBind) maps modalities to a joint space, but contrastive models only learn co-occurrence, not causality. ImageBind knows "dog + barking," but it doesn't know "dog's mouth is currently opening."
The Shift (Your Paper): We argue that true synchronization evaluation requires Fine-Grained Spatio-Temporal Semantic Reasoning. Only Omni-LLMs possess the world knowledge to understand that a visual action causes an acoustic consequence. We are upgrading synchronization from a low-level perception task to a high-level reasoning task.

3. To align Omni-LLMs with human perception of multimodal physics, we construct the first Multimodal Synchronization Preference Dataset. By leveraging 10 state-of-the-art Video-to-Audio models, we naturally map the distribution of current generative failures. We aren't just training an evaluator; we are training a Generative Reward Model. By applying a Bradley-Terry loss to human rankings, we force the Omni-LLM (Qwen-2.5 Omni) to distill its vast semantic knowledge into a continuous scalar representation of temporal-causal alignment.

4. The Problem: Traditional RL (like GRPO/PPO) in LLMs is designed for discrete token generation. How do you apply RL to a model acting as a continuous scalar evaluator?
The Innovation: We introduce a novel continuous-RL bridging technique. We reformulate the deterministic score regression as a Continuous Gaussian Policy (where the score is the mean, and the variance is manually parameterized). This brilliant abstraction allows us to apply GRPO—a highly efficient discrete-RL algorithm—directly to a continuous reward modeling task.
The Impact: This proves that Omni-LLMs can be self-improved via RL not just for chat, but as continuous sensory evaluators. It opens a massive new door for the RLHF community.

